Concentration of empirical barycenters in metric spaces

Barycenters (aka Fr\'echet means) were introduced in statistics in the 1940's and popularized in the fields of shape statistics and, later, in optimal transport and matrix analysis. They provide the most natural extension of linear averaging to non-Euclidean geometries, which is perhaps the most basic and widely used tool in data science. In various setups, their asymptotic properties, such as laws of large numbers and central limit theorems, have been established, but their non-asymptotic behaviour is still not well understood. In this work, we prove finite sample concentration inequalities (namely, generalizations of Hoeffding's and Bernstein's inequalities) for barycenters of i.i.d. random variables in metric spaces with non-positive curvature in Alexandrov's sense. As a byproduct, we also obtain PAC guarantees for a stochastic online algorithm that computes the barycenter of a finite collection of points in a non-positively curved space. We also discuss extensions of our results to spaces with possibly positive curvature.

==> biblio.tex <==
@book {Alexandrovgeom,
    AUTHOR = {Alexander, Stephanie and Kapovitch, Vitali and Petrunin,
              Anton},
     TITLE = {An invitation to {A}lexandrov geometry},
    SERIES = {SpringerBriefs in Mathematics},
      NOTE = {CAT(0) spaces},
 PUBLISHER = {Springer, Cham},
      YEAR = {2019},
     PAGES = {xii+88},
      ISBN = {978-3-030-05311-6; 978-3-030-05312-3},
   MRCLASS = {53C23 (51F99 53C20 53C45 53C70)},
  MRNUMBER = {3930625},
MRREVIEWER = {Loreno Heer},
       DOI = {10.1007/978-3-030-05312-3},
       URL = {https://doi.org/10.1007/978-3-030-05312-3},
}

@article {surveymetricentropy,
    AUTHOR = {Gin\'{e}, Evarist},
     TITLE = {Empirical processes and applications: an overview},
      NOTE = {With a discussion by Jon A. Wellner and a rejoinder by the
              author},
   JOURNAL = {Bernoulli},
  FJOURNAL = {Bernoulli. Official Journal of the Bernoulli Society for
              Mathematical Statistics and Probability},
    VOLUME = {2},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {1--38},
      ISSN = {1350-7265},
   MRCLASS = {60F17 (60F15 62G30)},
  MRNUMBER = {1394050},
MRREVIEWER = {Miguel A. Arcones},
       DOI = {10.2307/3318565},
       URL = {https://doi.org/10.2307/3318565},
}

@article{afsari2011riemannian,
  title={Riemannian $L^p$-center of mass: existence, uniqueness, and convexity},
  author={Afsari, Bijan},
  journal={Proceedings of the American Mathematical Society},
  volume={139},
  number={2},
  pages={655--673},
  year={2011}
}


@article{afsari2013convergence,
  title={On the convergence of gradient descent for finding the Riemannian center of mass},
  author={Afsari, Bijan and Tron, Roberto and Vidal, Ren{\'e}},
  journal={SIAM Journal on Control and Optimization},
  volume={51},
  number={3},
  pages={2230--2260},
  year={2013},
  publisher={SIAM}
}

@article{agueh2011barycenters,
  title={Barycenters in the Wasserstein space},
  author={Agueh, Martial and Carlier, Guillaume},
  journal={SIAM Journal on Mathematical Analysis},
  volume={43},
  number={2},
  pages={904--924},
  year={2011},
  publisher={SIAM}
}


@article{altschuler2021averaging,
  title={Averaging on the Bures-Wasserstein manifold: dimension-free convergence of gradient descent},
  author={Altschuler, Jason and Chewi, Sinho and Gerber, Patrik R and Stromme, Austin},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={22132--22145},
  year={2021}
}


@article{altschuler2021wasserstein,
  title={Wasserstein barycenters can be computed in polynomial time in fixed dimension.},
  author={Altschuler, Jason M and Boix-Adsera, Enric},
  journal={J. Mach. Learn. Res.},
  volume={22},
  pages={44--1},
  year={2021}
}

@article{altschuler2022wasserstein,
  title={Wasserstein barycenters are NP-hard to compute},
  author={Altschuler, Jason M and Boix-Adsera, Enric},
  journal={SIAM Journal on Mathematics of Data Science},
  volume={4},
  number={1},
  pages={179--203},
  year={2022},
  publisher={SIAM}
}

@incollection{bacak2014convex,
  title={Convex analysis and optimization in Hadamard spaces},
  author={Bac{\'a}k, Miroslav},
  booktitle={Convex Analysis and Optimization in Hadamard Spaces},
  year={2014},
  publisher={de Gruyter}
}

@article{bhatia2006riemannian,
  title={Riemannian geometry and matrix geometric means},
  author={Bhatia, Rajendra and Holbrook, John},
  journal={Linear algebra and its applications},
  volume={413},
  number={2-3},
  pages={594--618},
  year={2006},
  publisher={Elsevier}
}

@incollection{bhatia2009positive,
  title={Positive definite matrices},
  author={Bhatia, Rajendra},
  booktitle={Positive Definite Matrices},
  year={2009},
  publisher={Princeton university press}
}

@article{bhatia2019bures,
  title={On the Bures--Wasserstein distance between positive definite matrices},
  author={Bhatia, Rajendra and Jain, Tanvi and Lim, Yongdo},
  journal={Expositiones Mathematicae},
  volume={37},
  number={2},
  pages={165--191},
  year={2019},
  publisher={Elsevier}
}

@article{bhattacharya2003large,
  title={Large sample theory of intrinsic and extrinsic sample means on manifolds},
  author={Bhattacharya, Rabi and Patrangenaru, Vic},
  journal={Annals of statistics},
  volume={31},
  number={1},
  pages={1--29},
  year={2003},
  publisher={Institute of Mathematical Statistics}
}

@article{bhattacharya2005large,
  title={Large sample theory of intrinsic and extrinsic sample means on manifolds: {I}{I}},
  author={Bhattacharya, Rabi and Patrangenaru, Vic},
  journal={Annals of statistics},
  pages={1225--1259},
  year={2005},
  publisher={JSTOR}
}


@article{bhattacharya2017omnibus,
  title={Omnibus CLTs for {F}r{\'e}chet means and nonparametric inference on non-Euclidean spaces},
  author={Bhattacharya, Rabi and Lin, Lizhen},
  journal={Proceedings of the American Mathematical Society},
  volume={145},
  number={1},
  pages={413--428},
  year={2017}
}


@article{billera2001geometry,
  title={Geometry of the space of phylogenetic trees},
  author={Billera, Louis J and Holmes, Susan P and Vogtmann, Karen},
  journal={Advances in Applied Mathematics},
  volume={27},
  number={4},
  pages={733--767},
  year={2001},
  publisher={Elsevier}
}



@inproceedings{boria2020Frechet,
  title={{F}r{\'e}chet Mean Computation in Graph Space through Projected Block Gradient Descent},
  author={Boria, Nicolas and Negrevergne, Benjamin and Yger, Florian},
  booktitle={ESANN 2020},
  year={2020}
}



@book{bridson2013metric,
  title={Metric spaces of non-positive curvature},
  author={Bridson, Martin R and Haefliger, Andr{\'e}},
  volume={319},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@book{burago2022course,
  title={A course in metric geometry},
  author={Burago, Dmitri and Burago, Yuri and Ivanov, Sergei},
  volume={33},
  year={2022},
  publisher={American Mathematical Society}
}

@book{chavel2006riemannian,
  title={Riemannian geometry: a modern introduction},
  author={Chavel, Isaac},
  volume={98},
  year={2006},
  publisher={Cambridge university press}
}

@inproceedings{chewi2020gradient,
  title={Gradient descent algorithms for {B}ures-{W}asserstein barycenters},
  author={Chewi, Sinho and Maunu, Tyler and Rigollet, Philippe and Stromme, Austin J},
  booktitle={Conference on Learning Theory},
  pages={1276--1304},
  year={2020},
  organization={PMLR}
}


@inproceedings{claici2018stochastic,
  title={Stochastic wasserstein barycenters},
  author={Claici, Sebastian and Chien, Edward and Solomon, Justin},
  booktitle={International Conference on Machine Learning},
  pages={999--1008},
  year={2018},
  organization={PMLR}
}


@inproceedings{cuturi2014fast,
  title={Fast computation of Wasserstein barycenters},
  author={Cuturi, Marco and Doucet, Arnaud},
  booktitle={International conference on machine learning},
  pages={685--693},
  year={2014},
  organization={PMLR}
}


@article{eltzner2019stability,
  title={Stability of the Cut Locus and a Central Limit Theorem for {F}réchet Means of {R}iemannian Manifolds},
  author={Eltzner, Benjamin and Galaz-Garcia, Fernando and Huckemann, Septhan F and Tuschmann, Wilderich},
  journal={arXiv preprint arXiv:1909.00410},
  year={2019}
}

@article{eltzner2019smeary,
  title={{A smeary central limit theorem for manifolds with application to high-dimensional spheres}},
  author={Eltzner, Benjamin and Huckemann, Stephan F},
  journal={The Annals of Statistics},
  volume={47},
  number={6},
  pages={3360--3381},
  year={2019},
  publisher={Institute of Mathematical Statistics}
}



@article {Frechet48,
    AUTHOR = {Fr\'{e}chet, Maurice},
     TITLE = {Les \'{e}l\'{e}ments al\'{e}atoires de nature quelconque dans un espace
              distanci\'{e}},
   JOURNAL = {Ann. Inst. H. Poincar\'{e}},
  FJOURNAL = {Annales de l'Institut Henri Poincar\'{e}},
    VOLUME = {10},
      YEAR = {1948},
     PAGES = {215--310},
      ISSN = {0365-320X},
   MRCLASS = {60.0X},
  MRNUMBER = {27464},
MRREVIEWER = {J. L. Doob},
       URL = {http://www.numdam.org/item?id=AIHP_1948__10_4_215_0},
}


@article{hotz2013sticky,
  title={Sticky central limit theorems on open books},
  author={Hotz, Thomas and Skwerer, Sean and Huckemann, Stephan and Le, Huiling and Marron, J Stephen and Mattingly, Jonathan C and Miller, Ezra and Nolen, James and Owen, Megan and Patrangenaru, Vic},
  journal={Annals of Applied Probability},
  year={2013}
}

@article{karcher1977Riemannian,
  title={{R}iemannian center of mass and mollifier smoothing},
  author={Karcher, Hermann},
  journal={Communications on pure and applied mathematics},
  volume={30},
  number={5},
  pages={509--541},
  year={1977},
  publisher={Wiley Online Library}
}


@book{kendall2009shape,
  title={Shape and shape theory},
  author={Kendall, David George and Barden, Dennis and Carne, Thomas K and Le, Huiling},
  volume={500},
  year={2009},
  publisher={John Wiley \& Sons}
}


@article{kendall2011limit,
  title={Limit theorems for empirical {F}r{\'e}chet means of independent and non-identically distributed manifold-valued random variables},
  author={Kendall, Wilfrid S and Le, Huiling},
  journal={Brazilian Journal of Probability and Statistics},
  volume={25},
  number={3},
  pages={323--352},
  year={2011},
  publisher={Brazilian Statistical Association}
}

@inproceedings{kroshnin2019complexity,
  title={On the complexity of approximating Wasserstein barycenters},
  author={Kroshnin, Alexey and Tupitsa, Nazarii and Dvinskikh, Darina and Dvurechensky, Pavel and Gasnikov, Alexander and Uribe, Cesar},
  booktitle={International conference on machine learning},
  pages={3530--3540},
  year={2019},
  organization={PMLR}
}

@article{kroshnin2021statistical,
  title={Statistical inference for Bures--Wasserstein barycenters},
  author={Kroshnin, Alexey and Spokoiny, Vladimir and Suvorikova, Alexandra},
  journal={The Annals of Applied Probability},
  volume={31},
  number={3},
  pages={1264--1298},
  year={2021},
  publisher={Institute of Mathematical Statistics}
}

@article{kubo1980means,
  title={Means of positive linear operators},
  author={Kubo, Fumio and Ando, Tsuyoshi},
  journal={Mathematische Annalen},
  volume={246},
  number={3},
  pages={205--224},
  year={1980},
  publisher={Springer}
}


@book {Ledouxconcentration,
    AUTHOR = {Ledoux, Michel},
     TITLE = {The concentration of measure phenomenon},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {89},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2001},
     PAGES = {x+181},
      ISBN = {0-8218-2864-9},
   MRCLASS = {28C15 (28A35 46B09 60E15 82B44)},
  MRNUMBER = {1849347},
MRREVIEWER = {Werner Linde},
       DOI = {10.1090/surv/089},
       URL = {https://doi.org/10.1090/surv/089},
}


@article{le2017existence,
  title={Existence and consistency of Wasserstein barycenters},
  author={Le Gouic, Thibaut and Loubes, Jean-Michel},
  journal={Probability Theory and Related Fields},
  volume={168},
  number={3},
  pages={901--917},
  year={2017},
  publisher={Springer}
}

@article{LimPalfia14,
author = {Lim, Yongdo and Pálfia, Miklós},
year = {2014},
month = {05},
pages = {},
title = {Weighted deterministic walks for the least squares mean on Hadamard spaces},
volume = {46},
journal = {Bulletin of the London Mathematical Society},
doi = {10.1112/blms/bdu008}
}


@inproceedings{massart2019curvature,
  title={Curvature of the manifold of fixed-rank positive-semidefinite matrices endowed with the Bures--Wasserstein metric},
  author={Massart, Estelle and Hendrickx, Julien M and Absil, P-A},
  booktitle={Geometric Science of Information: 4th International Conference, GSI 2019, Toulouse, France, August 27--29, 2019, Proceedings},
  pages={739--748},
  year={2019},
  organization={Springer}
}

@article {ohtapalfia,
    AUTHOR = {Ohta, Shin-ichi and P\'{a}lfia, Mikl\'{o}s},
     TITLE = {Discrete-time gradient flows and law of large numbers in
              {A}lexandrov spaces},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {54},
      YEAR = {2015},
    NUMBER = {2},
     PAGES = {1591--1610},
      ISSN = {0944-2669},
   MRCLASS = {53C23 (49L20 49M37 58C05)},
  MRNUMBER = {3396425},
MRREVIEWER = {Takumi Yokota},
       DOI = {10.1007/s00526-015-0837-y},
       URL = {https://doi.org/10.1007/s00526-015-0837-y},
}

@article {Funano10,
    AUTHOR = {Funano, Kei},
     TITLE = {Rate of convergence of stochastic processes with values in
              {$\R$}-trees and {H}adamard manifolds},
   JOURNAL = {Osaka J. Math.},
  FJOURNAL = {Osaka Journal of Mathematics},
    VOLUME = {47},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {911--920},
      ISSN = {0030-6126},
   MRCLASS = {60F05 (58J65 60B05)},
  MRNUMBER = {2791571},
MRREVIEWER = {Longmin Wang},
       URL = {http://projecteuclid.org/euclid.ojm/1292854310},
}

@book{simon2019loewner,
  title={Loewner's Theorem on Monotone Matrix Functions},
  author={Simon, Barry},
  year={2019},
  publisher={Springer}
}

@Article{Troyanov,
author = {M. Troyanov},
title = {Concentration et inégalité de {P}oincaré},
journal = {Séminaire Borel 2001 (IIIème Cycle Romand de Mathématiques).  Berne},
year = {2001},
OPTorganization = {Séminaire Borel 2001 (IIIème Cycle Romand de Mathématiques).  Berne},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}



@book{surveyineg,
    AUTHOR = {An\'{e}, C\'{e}cile and Blach\`ere, S\'{e}bastien and Chafa\"{\i}, Djalil and
              Foug\`eres, Pierre and Gentil, Ivan and Malrieu, Florent and
              Roberto, Cyril and Scheffer, Gr\'{e}gory},
     TITLE = {Sur les in\'{e}galit\'{e}s de {S}obolev logarithmiques},
    SERIES = {Panoramas et Synth\`eses [Panoramas and Syntheses]},
    VOLUME = {10},
      NOTE = {With a preface by Dominique Bakry and Michel Ledoux},
 PUBLISHER = {Soci\'{e}t\'{e} Math\'{e}matique de France, Paris},
      YEAR = {2000},
     PAGES = {xvi+217},
      ISBN = {2-85629-105-8},
   MRCLASS = {46N20 (26D15 46E99 58J60 60J10 60J60)},
  MRNUMBER = {1845806},
MRREVIEWER = {Emmanuel Russ},
}


@incollection {sturm03,
    AUTHOR = {Sturm, Karl-Theodor},
     TITLE = {Probability measures on metric spaces of nonpositive
              curvature},
 BOOKTITLE = {Heat kernels and analysis on manifolds, graphs, and metric
              spaces ({P}aris, 2002)},
    SERIES = {Contemp. Math.},
    VOLUME = {338},
     PAGES = {357--390},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2003},
   MRCLASS = {60B05 (28C15 28C99 53C21)},
  MRNUMBER = {2039961},
MRREVIEWER = {Vladimir I. Bogachev},
       DOI = {10.1090/conm/338/06080},
       URL = {https://doi.org/10.1090/conm/338/06080},
}



@article {fastconv,
    AUTHOR = {Le Gouic, T. and Paris, Q. and Rigollet, P. and Stromme, A.J.},
     TITLE = {Fast convergence of empirical barycenters in {A}lexandrov spaces and the {W}asserstein space},
   JOURNAL = {J. Eur. Math. Soc. },
      YEAR = {2022},
       DOI = {10.4171/jems/1234},
       URL = {https://doi.org/10.4171/jems/1234},
}

@article {convrate,
    AUTHOR = {Ahidar-Coutrix, A. and Le Gouic, T. and Paris, Q.},
     TITLE = {Convergence rates for empirical barycenters in metric spaces:
              curvature, convexity and extendable geodesics},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {177},
      YEAR = {2020},
    NUMBER = {1-2},
     PAGES = {323--368},
      ISSN = {0178-8051},
   MRCLASS = {60B05 (51F99 51K10 60B10 62G05)},
  MRNUMBER = {4095017},
       DOI = {10.1007/s00440-019-00950-0},
       URL = {https://doi.org/10.1007/s00440-019-00950-0},
}

@article {Ohtaconvexity,
    AUTHOR = {Ohta, Shin-ichi},
     TITLE = {Convexities of metric spaces},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {125},
      YEAR = {2007},
     PAGES = {225--250},
      ISSN = {0046-5755},
   MRCLASS = {53C21 (46E35 58E20)},
  MRNUMBER = {2322550},
MRREVIEWER = {Jeremy T. Tyson},
       DOI = {10.1007/s10711-007-9159-3},
       URL = {https://doi.org/10.1007/s10711-007-9159-3},
}

@incollection{Eltzner2021,
    AUTHOR = {Tran, Do and Eltzner, Benjamin and Huckemann, Stephan},
     TITLE = {Smeariness {B}egets finite sample smeariness},
 BOOKTITLE = {Geometric science of information},
    SERIES = {Lecture Notes in Comput. Sci.},
    VOLUME = {12829},
     PAGES = {29--36},
 PUBLISHER = {Springer, Cham},
      YEAR = {[2021]},
   MRCLASS = {60E05 (62R30)},
  MRNUMBER = {4424306},
       DOI = {10.1007/978-3-030-80209-7\_4},
       URL = {https://doi.org/10.1007/978-3-030-80209-7_4},
}


@book{vershynin2018high,
  title={High-dimensional probability: An introduction with applications in data science},
  author={Vershynin, Roman},
  volume={47},
  year={2018},
  publisher={Cambridge university press}
}


@article {Yokota16,
    AUTHOR = {Yokota, Takumi},
     TITLE = {Convex functions and barycenter on {CAT}(1)-spaces of small
              radii},
   JOURNAL = {J. Math. Soc. Japan},
  FJOURNAL = {Journal of the Mathematical Society of Japan},
    VOLUME = {68},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {1297--1323},
      ISSN = {0025-5645},
   MRCLASS = {53C23},
  MRNUMBER = {3523548},
MRREVIEWER = {Bo\.{z}ena Pi\polhk atek},
       DOI = {10.2969/jmsj/06831297},
       URL = {https://doi.org/10.2969/jmsj/06831297},
}

@article {Yokota18,
    AUTHOR = {Yokota, Takumi},
     TITLE = {Convex functions and {$p$}-barycenter on {${\rm
              CAT}(1)$}-spaces of small radii},
   JOURNAL = {Tsukuba J. Math.},
  FJOURNAL = {Tsukuba Journal of Mathematics},
    VOLUME = {41},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {43--80},
      ISSN = {0387-4982},
   MRCLASS = {53C23},
  MRNUMBER = {3705774},
MRREVIEWER = {Bo\.{z}ena Pi\polhk atek},
       DOI = {10.21099/tkbjm/1506353559},
       URL = {https://doi.org/10.21099/tkbjm/1506353559},
}

@inproceedings{zhang2016first,
  title={First-order methods for geodesically convex optimization},
  author={Zhang, Hongyi and Sra, Suvrit},
  booktitle={Conference on Learning Theory},
  pages={1617--1638},
  year={2016},
  organization={PMLR}
}

@article{zhang2018towards,
  title={Towards Riemannian accelerated gradient methods},
  author={Zhang, Hongyi and Sra, Suvrit},
  journal={arXiv preprint arXiv:1806.02812},
  year={2018}
}

@inproceedings{ziezold1977expected,
  title={On expected figures and a strong law of large numbers for random elements in quasi-metric spaces},
  author={Ziezold, Herbert},
  booktitle={Transactions of the Seventh Prague Conference on Information Theory, Statistical Decision Functions, Random Processes and of the 1974 European Meeting of Statisticians},
  pages={591--602},
  year={1977},
  organization={Springer}
}
